Green Operations of SWIPT Networks: The Role of End-User Devices

Internet of Things (IoT) devices often come with batteries of limited capacity that are not easily replaceable or rechargeable, and that constrain significantly the sensing, computing, and communication tasks that they can perform. The Simultaneous Wireless Information and Power Transfer (SWIPT) paradigm addresses this issue by delivering power wirelessly to energy-harvesting IoT devices with the same signal used for information transfer. For their peculiarity, these networks require specific energy-efficient planning and management approaches. However, to date, it is not clear what are the most effective strategies for managing a SWIPT network for energy efficiency. In this paper, we address this issue by developing an analytical model based on stochastic geometry, accounting for the statistics of user-perceived performance and base station scheduling. We formulate an optimization problem for deriving the energy optimal configuration as a function of the main system parameters, and we propose a genetic algorithm approach to solve it. Our results enable a first-order evaluation of the most effective strategies for energy-efficient provisioning of power and communications in a SWIPT network. We show that the service capacity brought about by users brings energy-efficient dynamic network provisioning strategies that radically differ from those of networks with no wireless power transfer.

==> 07.Simulator_implementation.tex <==
\subsection{Simulations}
\label{app:Simulations}

The simulator assumes that base stations work at full utilization. Thus, both in uplink and in downlink, they use all of their time to serve users, and what we measure is the \textit{ideal} per-bit and per-joule delay.\\
Computation of per-bit delay. 
For every base station i, for every user served in that base station, $N_u$ and $N_d$ are the number of broadband and IoT users served by that base station, respectively.\\
For the downlink:
\be\label{eq:taubroadband}
\tau_d(x)=\frac{N_u+\frac{\delta_d}{1-\eta}N_d}{C(x,P_{BS},G)}
\ee

If he is an IoT user, the ideal per-bit delay perceived is 

\[
\tau_{d,I}(x)=\frac{N_u+\frac{\delta_d}{1-\eta}N_d}{\delta_d C(x,P_{BS},G)}
\]
The script has to compute the average of these quantities across the whole area. In the average, every user is weighed by the relative size of the area served by the base station to which he is associated, with respect to the whole simulation area. 

Similarly, for the uplink we have 

\be\label{eq:taubroadband}
\tau_u(x)=\frac{N_u+\delta_u N_d}{C(x,P_{bb},1)}
\ee

and 
\[
\tau_{u,I}(x)=\frac{\tau_u(x)}{\delta_u}=\frac{N_u+\delta_u N_d}{\delta_u C(x,P_{I},1)}
\]

Same considerations as before hold here for averages.
As for per-joule delay, for each IoT user we compute
\begin{equation*}
  h(x)=\frac{1}{\xi}\Bigg\{P_{BS} D(x)^{-\alpha}\left[G K(x)+L\left(1-K(x)\frac{(1-\eta)}{\eta}\right)\right]+\bigg.
 \end{equation*}
\be
\left. +\left(1-K(x)\frac{(1-\eta)}{\eta}\right)(I(D(x),1) +H(x))\right\}^{-1}
\ee
with 
\[
K(x)=\frac{\frac{\delta_d\eta}{1-\eta}}{N_u+\frac{\delta_d}{1-\eta} N_d}
\]

A good way to compute the interfering power for a user at x is as follows. Let j be the label of the j-th base station. Then  
\[
I(D(x),k)=\frac{\sum_j P_{BS}D(x)^{-\alpha}L}{k}
\]
and 
\[
I_T(D(x))=k I(D(x),k)
\]
Computation of $H(x)$: Integrating over all users is overkill. What I can propose is as follows.
For every base station $j$:\\
-compute the center of gravity of that cell, $x_{c,j}$, i.e. the average of the coordinates of all users in that cell, and the distance between
$x_{c,j}$ and the user at $x$, that we denote $d(x_{c,j},x)$.
Given that $N_{u,j}$ and $N_{d,j}$ are the number of broadband and IoT users in cell $j$, we have then
\[
H(x)=\frac{\sum_j (N_{u,j} P_{bb}+\delta_u N_{d,j} P_{I})d(x_{c,j},x)^{-\alpha}L}{N_{u,j}+\delta_u N_{d,j}}
\]


==> 09.forjournalversion.tex <==

\subsection{Proof of \thref{th:BE_tau_stdev}}
\label{app:proof_stdev}
For the derivation of the mean harvested power, we need to compute $E^0[h(x)]$, where $h(x)$ is given by \lref{lemma:perjouledelay}.
Let $h(x)=F(x)+X(x)$, with:
\[
F(x)=\xi\{P_{BS} D(x)^{-\alpha}LU_d(x) +(kI(D(x),k) +O(x))\}
\]

\[
X(x)=\xi K(x)\left\{P_{BS} D(x)^{-\alpha}\left(G-\frac{L}{\eta}\right)\right.
\]

\[
\left . -\frac{1-\eta}{\eta}\left(k I(D(x),k) +O(x)\right)\right\}=\xi K(x)Z(x)
\]
Following the same procedure as in the previous derivation, we have
\[
E^0[F(D)| r \leq D \leq r + d r]=F(r)  
\]
while for $X(x)$ we have 
\[
E^0\left[X(D)| r \leq D \leq r + d r \right]= 
\]
\[
=\xi E^0\left[ K(D)| r \leq D \leq r + d r \right] Z(r)
\]
Using the notation of the proof of \thref{th:BE_tau}, we have that
\[
E^0\left[ K(D)| r \leq D \leq r + d r \right]=
\]
\[
=E^0\left[\frac{U_d(D)\eta}{1-\gamma(1-\delta_d(1-\eta))]N_{tot}(D)}| r \leq D \leq r + d r \right]
\]
where with $U_d(D)$ we denote the downlink utilization of the base station to which the user at the origin is associated.
We approximate the above expression, by substituting to $U_d(D)$ its mean value $\frac{\bar{\tau}_d}{\tau_0}$.
\[
=\frac{\bar{\tau}_d}{\tau_0}[1-\gamma(1-\delta_d(1-\eta))]\eta E^0\left[\frac{1}{N_{tot}(D)}| r \leq D \leq r + d r \right]
\]
As pointed out in the proof of \thref{th:BE_tau}, the random variable at the denominator is Poisson with intensity given by \eref{Eq:CondExp}.















\subsection{Old derivation}
AS there is no closed form exact formula for the pdf of the amount of users in a Voronoi cell, we resort to the following approximation. 
Let us rewrite the denominator in the expression of $h(x)$ as the sum of two terms, given by:
\[
F(x)=\xi\{P_{BS} D(x)^{-\alpha}LU_d +(kI(D(x),k) +O(x))\}
\]

\[
B(x)=\xi K(x)\left\{P_{BS} D(x)^{-\alpha}\left(G-\frac{L}{\eta}\right)\right.
\]

\[
\left . -\frac{1-\eta}{\eta}\left(k I(D(x),k) +O(x)\right)\right\}
\]

Following the same procedure as in the previous derivation,  we have

\[
%E^0[A(x)]=\int_0^{\infty} A(r) e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r d r$} 
E^0[F(D)| r \leq D \leq r + d r]=F(r)  
\]

\[
E^0\left[\frac{1}{B(D)}| r \leq D \leq r + d r \right]= 
\]
\[
=\frac{E^0[N_{iot}(r)+\delta_d(1-\eta(r)) N_{bb}(r)]}{\xi\eta[P_{BS} r^{-\alpha}(G-\frac{1-\eta}{\eta}L) -\frac{1-\eta}{\eta}(kI(r,k) +O(r))]\frac{\bar{\tau}_d}{\tau_d^0}}
\]
\[
=\frac{E^0[N_{iot}(r)+\delta_d(1-\eta(r)) N_{bb}(r)]}{\xi[P_{BS} r^{-\alpha}(G\eta-(1-\eta)L) -(1-\eta)(kI(r,k) +O(r))]\frac{\bar{\tau}_d}{\tau_d^0}}
\]

\[
=\frac{[1-\gamma(1-\delta_d(1-\eta))]\lambda_u\int_0^{\infty} \int_0^{2 \pi}  e^{- \lambda_b A(r, x, \theta)} d \theta x d x}{\xi[P_{BS} r^{-\alpha}(G\eta-(1-\eta)L) -(1-\eta)(kI(r,k) +O(r))]\frac{\bar{\tau}_d}{\tau_d^0}} =\frac{1}{X(r)}
\]
Using Jensen's inequality, a conservative estimate of the the mean harvested power is thus given by 

\begin{equation}
\int_0^{\infty} (F(r)+X(r))e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \diff r.
\end{equation}

%The approximation here consists in assuming that the user is harvesting energy from ambient sources (i.e. from signal sent by the base station serving it to the other users, as well as by other base stations and by users) even when receiving information from its serving base station.
% The rest of the derivation of \eref{eq:perjoule2} follows along the same lines as \eref{eq:Poisson}.
% Finally, the system of equations (\ref{eq:system}) is derived from imposing that conditions (\ref{eq:cond1}) and (\ref{eq:cond2}) hold for the palm expectations, i.e. 
% \[
% \frac{\bar{h}}{h_0}=\frac{\bar{\tau}}{\tau_0}=\bar{U}
% \]
%\com{se questa non va c'e' un approx che consiste in un problema di punto fisso, che consiste nel calcolare il n medio di utenti per cella voronoi in modo indipendente e poi sostituire. questo consiste nell'ignorare la correlazione...}




Let $h(x)$ be the mean harvested power by a user at $x$. By the definition of variance,
\com{sviluppa}
\[
V^0[h(x)]= E^0[h^2(x)]-(E^0[h(x)])^2 =E^0[h^2(x)] - \bar{h}^2
\]
 The derivation of $E^0[h^2(x)]$ follows along the same lines as the one for $E^0[h(x)]$.
 
 \[
 E^0[h^2(x)] =
 \]
\be\scalebox{0.8}[1]{$= \int_0^{\infty}  \frac{E^0[(N_{bb}(S(0))+\frac{\delta_d}{1-\eta(S(0))} N_{iot}(S(0)))^2| r \leq D(0) \leq r + d r ]}{D^2(r)}e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r d r$} \ee
The conditional expectation within the integral becomes 
\begin{eqnarray*}%\qquad \qquad \quad
&=& E^0\Bigg[\lambda^2_u\left(\int_0^{\infty} \int_0^{2 \pi} \mathbf{1}_{(S(x,\theta) = S(0)| r \leq D(0) \leq r + d r)} d \theta x d x\right)^2 \Bigg]\\
& &\left(1-\gamma\left(1-\frac{\delta_d}{1-\eta}\right)\right)^2\\
&=&\lambda^2_u\left(\int_0^{\infty} \int_0^{2 \pi} e^{- \lambda_b A(r, x, \theta)} d \theta x d x\right)^2 \left(1-\gamma\left(1-\frac{\delta_d}{1-\eta}\right)\right)^2\\
\end{eqnarray*}
Substituting,
\[
 E^0[h^2(x)] =\int_0^{\infty} f^2(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{D^2(r,\eta)}   \diff r
 \]
and the standard deviation of $h(x)$ is thus
\be
\sigma_h=\sqrt{\int_0^{\infty} f^2(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{D^2(r,\eta)}   \diff r- \bar{h}}
\ee

\begin{table}[th!]
\vspace{2mm}
\caption{Main notation used in the paper.}
%\centering % to have the caption near the table
\footnotesize
\begin{tabular}{p{0.15\columnwidth} | p{0.7\columnwidth}}
%\toprule 
Notation &  Parameter \\
\hline
$\lambda_{b}$ &  Mean base station density ($m^{-2}$)\\

%\bottomrule
\end{tabular}
\normalsize
\label{tab:TableOfNotation}
\end{table}

In realistic settings, better frequency management mechanisms can be implemented, which minimize the probability of two neighboring cells sharing the same frequency band. However, with probabilistic sleep modes, random reuse allows keeping such probability independent of the density of active BSs, and hence it allows estimating the impact of interference on energy saving strategies independently of any frequency management mechanism.


\textbf{IoT user}: For an IoT user in $x$ in the active state, the power consumed is   
\vspace{-0.2in}
\be\label{eq:energymodel_iot}
R_{iot,A}(x)=w_1 + w_2 U_{I}(x)P_{I} 
\ee
where $w_1$ models the mean power consumed when the device is not transmitting (we assume receiving traffic does not impact significatively power consumption)

\begin{itemize}
    %\item $U(S(x))$ is the utilization of the base station to which the user is associated;
    % \item $U_{cpu}$ is the mean CPU utilization, and $w_2 U_{cpu}$ accounts for the mean power consumed by computing tasks;
    \item $U_{I}$ is the mean fraction of time the user is busy transmitting, and $P_{I}$ is the transmit power of the device. Thus $w_2 U_{I}P_{I}$ models the mean power consumed due to signal transmission. 
    %\com{Either we let $U_{I}=1$, or we make it a function of how many users are served at the base station, i.e. $U_{I}=U_{I}(x)$.}
    \item $w_1$ models all those contributions to mean consumed power which do not depend on $U_{I}$ or $P_{I}$.
    %\item $\tilde{h}(x)$ is the per-Joule delay perceived by the user, and thus $\frac{1}{\tilde{h}(x)}$ is the mean power harvested by the device. 
\end{itemize} 
In the low power state instead, the power consumed is equal to a constant, denoted with $w_l$, which we assume to be inferior to $w_1$.
%Equation \eref{eq:energymodel_iot} describes the overall mean rate at which the energy available for an IoT device varies over time. Thus, a necessary condition for a device in $x$ to be available (i.e. to have on average, enough power for its operations) is to have $R_{iot}(x)\geq 0$).



\textbf{As a consequence of the definition of $\delta_{j}$, the target values of per bit delay for IoT users are $\delta_{j}$ times those for BB users}. Indeed, given that IoT and BB UEs are both distributed uniformly at random in space, the difference between their expected per bit delay will be given only by the difference between the duration of the BS time dedicated to UEs from each of the two classes, i.e. $\delta_d$ and $\delta_u$.\\


Specifically, let us consider a UE located at the origin. The BS with which it is associated (located in $S(0)$) sets $\beta_d=\beta^*_d$, where $\beta^*_d$ is the solution of the following equation:
\[
\frac{1}{N_{bb}(S(0))+N_{iot}(S(0))}\left (\sum_{x\in\mathcal{X}_{bb}}\tau_d^{id}(x)\mathbf{1}_{S(x) = S(0)}+\right .
\]
\begin{equation}\label{eq:cond1}
\left .+\delta_d\sum_{x\in\mathcal{X}_{iot}}\tau_{d,I}^{id}(x)\mathbf{1}_{S(x) = S(0)}\right)\frac{1}{\tau_d^0} = U_d(S(0))
\end{equation} 
% \begin{equation*}
% \frac{\sum_{x\in\mathcal{X}_d}\tau_d(x)}{N_d(S(x))}\mathbf{1}_{S(x) = S(0)} =\bar{\tau}_{d}^0U(S(0))
% \end{equation*} 
% \begin{equation}\label{eq:cond2}
% \frac{1}{h_0}\sum_{x\in\mathcal{X}_d}\frac{h(x)}{N_{iot}(S(x))}\mathbf{1}_{S(x) = S(0)} = U(S(0))
% \end{equation}
% \[
% \frac{1}{N_{bb}(S(0))+N_{iot}(S(0))}\left (\sum_{x\in\mathcal{X}_{u}}\tau_u(x)\mathbf{1}_{S(x) = S(0)}+\right .
% \]
% \begin{equation}\label{eq:cond1}
% \left .+\delta_u\sum_{x\in\mathcal{X}_{d}}\tau_{u,I}(x)\mathbf{1}_{S(x) = S(0)}\right)\frac{1}{\tau_u^0} = U_u(S(0))
% \end{equation} 
where $\tau_{d,I}^{id}$ is the ideal per-bit delay perceived by IoT users, $\mathcal{X}_{bb}$ and $\mathcal{X}_{iot}$ are the set of broadband and of IoT users, respectively, and the $U_d$ are given by \eref{eq_utilization}. A similar expression holds for $\beta_u$, where per bit delays are measured when IoT devices are in active state.

\com{By the GPS scheduling, the mean throughput of the user at $x$ is obtained by dividing the capacity $C(r,P_{BS},G,I)$ seen by that user by the sum of the GPS weight of all the users associated with that BS (including both BB and IoT users) and of $\beta_{d}$,
%\footnote{this is just normalization}, 
and multiplying the result by the GPS weight of the class of users that the user at $x$ belongs to.}

In settings with dense small cells, it becomes crucial to model accurately the effect of interference on user perceived performance. In order to do so, it is essential to model its dependency on traffic patterns. In what follows, we propose a result which relates the main performance indicators to  system parameters, such as user density, BS density, and the target QoS values for the network, in terms of expected per-bit and per-joule delays.


\begin{lemma}\label{lemma:user_utilization} The mean fraction of time spent transmitting by an IoT user is given by 
\be
\bar{U}_{I}=\frac{1 }{\delta_uH(\frac{\delta_u}{\phi},0,1 )}\frac{\bar{\tau}_u}{\tau^0_u}
\ee
\end{lemma}

\begin{proof} The fraction of time spent transmitting by an IoT user located at $x$ is given by
\be
U_I(x)=\frac{1}{\phi N_{iot}(S(x))+\delta_u N_{bb}(S(x))+\beta_u}
\ee
\[
=\frac{1}{\phi N_{iot}(S(x))+\delta_u N_{bb}(S(x))}U_u(S(x))
\]
where with $U_u(S(x))$ we denote the BS utilization in uplink, for the BS which is serving the IoT user at x.
We approximate $U_u(S(x))$ with its expected value $\frac{\bar{\tau}_u}{\tau^0_u}$.
We have therefore
\be
E^0[U_I(x)]=E^0\left[\frac{1}{\phi N_{iot}(S(x))+\delta_u N_{bb}(S(x))}\right]\frac{\bar{\tau}_u}{\tau^0_u}
\ee
We introduce a second approximation, computing the expectation of the inverse as the inverse of the expectation (Jensen's inequality, tight when the number of users is high). We get:
\[
\geq \frac{1}{E^0\left[\phi N_{iot}(S(x))+\delta_u N_{bb}(S(x))\right]}\frac{\bar{\tau}_u}{\tau^0_u}
\]
\[
=\frac{1}{\delta_u H(\frac{\delta_u}{\phi},0, 1)}\frac{\bar{\tau}_u}{\tau^0_u}
\]
%\frac{\bar{\tau}_u}{\tau^0_u}
\end{proof}

\begin{theorem}\label{corollary_recharging} For the typical user arriving in the system at a distance $r$ from the serving BS, the power harvesting is not sufficient when the following inequality holds:
\[
F(r)+\frac{X(r)}{f(r,\eta,\delta_d)}< cycle*(w_1+w_2U_{cpu}+w_3U_I(r)P_I)
\]
where 
\[
U_I(r)=\frac{1}{\phi f\left(r,0,\frac{\delta_u}{\phi} \right)}
\]
\end{theorem}
Thus, let 
\[
Q(r)=F(r)+\frac{X(r)}{f(r,\eta,\delta_d)}-cycle*(w_1+w_2U_{cpu}+w_3U_I(r)P_I)
\]
Then, the probability for an IoT device of not harvesting a sufficient amount of power for its operation is given by $CDF_r(Q^{-1}(0))$. This takes into account both the correlation between amount of harvested energy and QoS perceived by the user, and the impact of user device utilization on consumed energy.


\bt\label{th:BE_tau_stdev} The mean power harvested by an IoT user who is just beginning service is given by

\begin{equation}
\bar{h}=\int_0^{\infty} \left(F(r)+\frac{X(r)}{f(r,\eta,\delta_d)}\right)e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \diff r.
\end{equation}
with 
\[
F(r)=\xi\left[P_{BS} r^{-\alpha}L\frac{\bar{\tau}_d}{\tau_d^0} +k\bar{I}(r,k) +\bar{O}\right]
\]
% \[
% X(r)=\frac{\xi[P_{BS} r^{-\alpha}(G\eta-(1-\eta)L) -(1-\eta)(k\bar{I}(r,k)+ \bar{O})]\frac{\bar{\tau}_d}{\tau_d^0}} {[1-\gamma(1-\delta_d(1-\eta))]\lambda_u\int_0^{\infty} \int_0\pi}  e^{- \lambda_b A(r, x, \theta)} d \theta x d x}
% \]
\[
X(r)=\xi\frac{\bar{\tau}_d}{\tau_d^0}\left[P_{BS} r^{-\alpha}(G\eta-L) -(1-\eta)(k\bar{I}(r,k)+ \bar{O})\right]
\]

While the variance is 
 \[
 \sigma_h^2=\int_0^{\infty} \left[F(r)^2+\frac{2X(r)}{f(r,\eta,\delta_d)}+\frac{X(r)^2}{f(r,\eta,\delta_d)^2+f(r,\eta,\delta_d)}\right]\cdot
 \]
 \be\label{eq:stdev}
 \cdot e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \diff r- \bar{h}^2
 \ee
 \et
 
 In the dense IoT regime (i.e. when the density of IoT users is high), the cumulative distribution function $CDF_h$ of the power harvested by an IoT user who is just beginning service is
 \[
 CDF_h(h_0)=CDF_r(g^{-1}(h_0))
 \]
 for all $h_0\geq 0$, where $CDF_r$ is the cumulative distribution function of the distance of the user to its serving BS, given by
  \[
 CDF_r(r)=\int_0^{r}e^{- \lambda_b \pi y^2} \lambda_b 2 \pi ydy
 \]
 and where 
 \[
 g(r)=F(r)+\frac{X(r)}{f(r,\eta,\delta_d)}
 \]
For the proof, please refer to \aref{app:proof_stdev}. 

\com{
\begin{itemize}
    \item Can we assume best-effort traffic (no guarantee other than the mean?)
\item Or guarantee a min service (i.e. constraint on CDF of per bit delay, easy to compute? joint CDF?)
\end{itemize}
}

The energy optimal network configuration derives from solving the following optimization problem:
\begin{problem}\label{Prob:Opt_1}
%\vspace{-0.05in}
%\label{eq:objectivefunction}
 \[
 min_{\lambda_b,P,\eta}\;\;\lambda_{b}\left[q_1 +\frac{\bar{\tau}_d(\lambda_b,P)}{\tau^0_d}\left(q_2+q_3(P-P_{BS,min})\right)\right]
 \]
%\vspace{-0.1in}
Subject to:
%\vspace{-0.1in}
	\begin{align}
	 \frac{\bar{\tau}_d}{\tau^0_d}\leq & 1\label{eq:constraint1_downlink}\\
\frac{\bar{\tau}_u}{\tau^0_u}\leq	&  1\label{eq:constraint1_uplink}\\
0\leq \lambda_b\leq 	& \lambda_{b,max}\label{eq:constraint2}\\
P_{BS,min}\leq P \leq 	& P_{BS,max}\label{eq:constraint3}\\
CDF_h(h_0)\leq 	& \mu \label{eq:constraint_charging}\\
	h_0 = & w_1 + w_2 U_{cpu} +w_3 \bar{U}_{I}P_{I}\label{eq:constraint_charging}
%& \bar{U}_{I}=\frac{\delta_u }{H(\delta_u,0,1 )}\frac{\bar{\tau}_u}{\tau^0_u}
	\end{align}
	%\vspace{-0.2in}
\end{problem}
%\textbf{modeling $P_T$ is important as the ``cost'' of $P_T$ is also due to interference}
%\begin{eqnarray}\bar{\tau}(\lambda_b,\lambda_u) =&& \int_0^{\infty} \left(\int_0^{\infty} \int_0^{2 \pi} 
%e^{- \lambda_b A(r, x, \theta)} \lambda_{u} x \d \theta \d x  \right)\nonumber\\
%&& \qquad \frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{C(r)}   \d r.
%\end{eqnarray} 
%The lower bound $\lambda_{b,min}$ to BS density is typically determined by the minimum SNR (SINR) acceptable at the receiver. 
The maximum BS density $\lambda_{b,max}$ is determined by practical, technical (backhaul technology) and economic considerations. 
We assume that the target per-bit delays in uplink and downlink, for both broadband and IoT users, and 
the minimum power $h_0$ required by each IoT device to operate, are given as well as the maximum acceptable ratio of IoT users which harvest less than $h_0$ Joules per second, denoted as $\mu$. 


% We first rewrite the fixed point problem as follows. Let  
% $\beta(\eta)=\left[1-\gamma\left(1-\frac{\delta_d}{1-\eta}\right)\right]$
% We note that the expressions of \thref{th:BE_tau} can be rewritten as
% \[
% \bar{N}(\eta) =\beta(\eta) \pi
% \]
% \[
% \bar{\tau}_d =\beta(\eta) \mu
% \]
% \[
% \bar{h} =\beta(\eta) \omega(\eta)
% \]

% Then we have that the system of equations takes the form
% \[
% \frac{\beta(\eta) \omega(\eta)}{h_0}=\frac{\beta(\eta) \mu}{\tau_0}
% \]
% and 
% \be\label{eq_deltaidle}
% \frac{\beta(\eta) \mu}{\tau_0}=\frac{\beta(\eta) \pi}{\beta(\eta) \pi+\bar{\delta}_{idle}}
% \ee
% Simplifying, we get:
% \be\label{eq_eta_implicit}
%  \omega(\eta)=\frac{\mu h_0}{\tau_0}
% \ee
% which gives the expression of $\eta$. Substituting into \eref{eq_deltaidle} we get the expression of $\bar{\delta}_{idle}$.
% \com{Domande: 1)quante soluzioni valide ha \eref{eq_eta_implicit}? Si puo' studiare come problema di punto fisso. In tal caso, ha un solo punto fisso?}


% \textbf{Prova vecchia!}
% In order to prove that \eref{eq:Poisson} has a unique fixed point, we have to prove that the operator 
% $T(\bar{\tau})$, whose expression is given by the right member of \eref{eq:Poisson}, is a contraction. To do so, we verify that Blackwell's sufficient conditions for a contraction \cite{blackwell1965discounted} hold for $T$. The monotonicity of $T$ is straightforward, as with increasing $\bar{\tau}$ increases the mean BS  utilization, and hence their interference. And this translates into an increase in per-bit delays computed in \eref{eq:Poisson}.\\
% For the discounting property, we have to prove that $\exists \beta\in(0,1)$ such that 
% \be\label{eq:contraction}
% T(\bar{\tau}+ a)\leq T(\bar{\tau})+\beta a
% \ee
% $\forall a \geq 0$ and for all system parameter values for which $\bar{\tau}$ is defined. 
% Using the expression for the operator $T(\bar{\tau})$ from \thref{th:XXX}, we have 

% \[T(\bar{\tau}+ a)-T(\bar{\tau})=\int_0^{\infty} \left(\int_0^{\infty} \int_0^{2 \pi} 
% e^{- \lambda_b A(r, x, \theta)} \lambda_{u} x \diff\theta \diff x  \right)\cdot
% \]
% \[
% \cdot e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \left(\frac{1}{C(r,\bar{\tau}+a)}-\frac{1}{C(r,\bar{\tau})}\right) \diff r
% \]
% Now we have 
% \[
% \frac{1}{C(r,\bar{\tau}+a)}-\frac{1}{C(r,\bar{\tau})}=
% \]
% \[
% =\frac{\log_{2}\left(\frac{1 + \frac{p r^{-\alpha}}{N_0+I(r,k,\bar{\tau})}}{1 + \frac{p r^{-\alpha}}{N_0+I(r,k,\bar{\tau}+a)}}\right)}{\frac{B}{k}\log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k,\bar{\tau})}\right)\log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k,\bar{\tau}+a)}}\right)}
% \]
% We have $I(r,k,\bar{\tau}+ a)=I(r,k,\bar{\tau})+I(r,k,a)$. Substituting, we have 
% \[
% =\frac{\log_{2}\left[\left(1+\frac{I(r,k,a)}{N_0+I(r,k,\bar{\tau})}\right)\left( 1+\frac{I(r,k,a)}{N_0+I(r,k,\bar{\tau})+p r^{-\alpha}}\right)  \right]}{C(r,\bar{\tau})\log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k,\bar{\tau}+a)}}\right)}
% \]




% \[
% (B/k) \log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k)+K a p r^{-\alpha}}\right)\geq
% \]
% \[
% \geq (B/k)\left[ \log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k)}\right)-\log_{2}\left(K a p r^{-\alpha} \right)\right]
% \]




% We apply the Taylor series expansion of $\frac{1}{c-x}$ for $x\rightarrow 0$ to the fraction at the integrand, and we have, for $a \rightarrow 0$ 
% \[
% \frac{1}{C(r,\bar{\tau})-(B/k)\log_{2}\left(K a p r^{-\alpha}\right)}\geq
%  \frac{1}{C(r,\bar{\tau})}+\frac{B\log_{2}\left(K a p r^{-\alpha}\right)}{kC^2(r,\bar{\tau})}
% \]
% %To prove the discounting property, we have to prove that 
% Now we have 
% \vspace{-0.2in}
% \be\label{eq:inequality1}
% (B/k)\frac{\log_{2}\left(K a p r^{-\alpha}\right)}{C(r,\bar{\tau})}\leq K a\frac{\log_{2}\left( p r^{-\alpha}\right)}{log_{2}\left(1 + \frac{p r^{-\alpha}}{N_0+I(r,k)}\right)}
% \ee
% By substituting in the expression %in \eref{eq:interference} 
% (\ref{eq:interfpower2}) for the interfering power, for $p\leq 20 W$, and $\lambda_b\leq 10^4$ $BS/km^2$, the right member in \eref{eq:inequality1}
% is upper bounded by $K\beta a$, with $0\leq \beta <1$. Hence $T(\bar{\tau}+ a)\leq T(\bar{\tau}) (1 + K \beta a)$, and as the utilization $U\leq 1$, 
% $T(\bar{\tau}+ a)\leq T(\bar{\tau}) + \beta a$, which proves the discounting property. Being $T(\bar{\tau})$ a contraction, by the Banach fixed point theorem, the fixed point problem in \eref{eq:Poisson} admits a unique solution.
% \end{proof}

% %%%%%UPLINK

% \begin{proof}\textbf{uplink}.
% $\bar{\beta}_{idle}$ is given by the solution of:
% \be\label{eq:system_uplink}
% \frac{\bar{\tau}_u}{\tau_0}=\frac{\bar{M}}{\bar{M}+\bar{\beta}_{idle}}
% \ee
% \end{proof}


% \subsection{Computing $E^0[\rho^V]$ and $V^0[\rho^V]$}
% \label{sec:momentComputation}
% We use Campbell's formula \cite{Stoyan1987} in the computations below.

% \subsubsection{Poisson Layout}
% \begin{eqnarray*}
% E^0[\rho^V] &=& E^0\big[\sum_{x \in \Pi_u} \frac{R_0}{C(|x|)} \mathbf{1}(S(x) = S(0))\big]\\
% &=& E\left[E^0[\sum_{x \in \Pi_u} \frac{R_0}{C(|x|)} \mathbf{1}(S(x) = S(0))|\sigma(\Pi_b)] \right]\\
% &=& E\bigg[\lambda_u \frac{\mu_H^{-1}}{\mu_H^{-1} + \mu_W^{-1}}\int_0^{2\pi} \int_0^\infty \frac{R_0}{C(r)} \\&&\mathbf{1}(S(x) = S(0)) r \d r \d \theta \bigg]\\
% &=& \lambda_u\frac{\mu_H^{-1}}{\mu_H^{-1} + \mu_W^{-1}} \int_0^{2\pi} \int_0^\infty \frac{R_0}{C(|x|)} \exp(-\lambda_b \pi r^2)\\&& r \d r \d \theta \\
% &=& 2 \pi \lambda_u \frac{\mu_H^{-1}}{\mu_H^{-1} + \mu_W^{-1}}R_0 \int_0^\infty \frac{1}{C(r)} \exp(-\lambda_b \pi r^2)\\&& r \d r.
% \end{eqnarray*}
% Similarly, we can derive
% \begin{eqnarray*}
% V^0[\rho^V] &=& 2 \pi \lambda_u \frac{\mu_H^{-1}}{\mu_H^{-1} + \mu_W^{-1}}\int_0^\infty \left(\frac{R_0}{C(r)}\right)^2\\&& \exp(-\lambda_b \pi r^2) r \d r.
% \end{eqnarray*}


\begin{lemma}\label{lemma_recharging} The average power received from users for the typical user arriving in the system at a distance $r$ from the serving BS is approximated by 
\vspace{-0.15in}
\be
\bar{O}=\frac{(1-\gamma)\delta_u P_{bb} +\phi \gamma P_I}{(1-\gamma)\delta_u+\phi\gamma}\frac{\lambda_b\pi \alpha }{\alpha-2}\frac{\bar{\tau}_u}{\tau_u^0}
\ee
\vspace{-0.08in}
%where $\bar{\tau}$ is the mean of the ideal expected per-bit delay.  
\end{lemma}
%Note that both \lref{lemma_interference} and \lref{lemma_recharging} give a conservative estimate, as they both assume that every user/BS has always data to transmit. 
An interesting feature emerging from \lref{lemma_recharging} is that the mean power received from other users does not depend on user density. 
\begin{proof}  
%\usepackage{}\com{We assume that users have always data to transmit in upload (saturated model). This model can be changed, e.g. by assuming that users have a given mean throughput demand in upload, so that getting more for them is like assuming they will be transmitting less often.}
Given the proportion of users which are IoT devices, and the ratio between the GPS weights of broadband and IoT users in uplink,
whenever a user is transmitting, the probability that it is a broadband user is given by
\be\label{eq:ratio}
\frac{(1-\gamma)\delta_u }{(1-\gamma)\delta_u+\gamma}
\ee
%and the 
Thus the mean transmit power from a user is given by 
\begin{equation*}
    \frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}
\end{equation*}
The power received at at time $t$ for a user at a location $x$ from a user at another location which is transmitting is a random variable, depending on the relative position of the two users, as well as on the specific uplink traffic pattern of the user.
Specifically, let $x'_i(t) , i\in\chi(j)$ be the position of the $i$-th user served by BS $j$ at time t, $d(x,x'_i(t))$ denote the distance between the two users considered, and $u(x'_i(t))$ the probability that the given user is transmitting at time $t$. Then we can write the expression of $O(x,t)$ as 
\be\label{eq:palminterf}
\sum_{j}\sum_{i\in\chi(j)}\frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}d(x,x'_i(t)) ^{-\alpha}u(x'_i(t))
\ee
%\vspace{-0.2in}
where $\chi(j)$ is the set of users served by BS j. 
% $u_i(t)$ is equal to $1$ if the $i-th$ user is transmitting at time $t$. 
% Note that neither the ratio between bb and IoT users nor the relative duration of the time that BS j dedicates to each of these two classes of users depend on j. Thus we can write 
% \begin{equation}
%     E[H(x,t)]=E\left[\frac{(N_{bb,j}P_{bb}+\delta_u N_{iot,j}P_I)}{(N_{bb,j}+\delta_d N_{iot,j})}\right]\cdot
% \end{equation}
% \[
% \cdot E\left[\sum_{j}\sum_{i\in\chi(j)}d(x,x'_j(t)) ^{-\alpha}u_{i}(t)\right]=
% \]
% and approximating the expectation of the fraction as the ratio of the expectations, we have 
% \begin{equation*}
%     =\frac{\gamma P_{bb}+\delta_u (1- \gamma)P_I}{\gamma+\delta_u (1-\gamma)}\cdot
% \end{equation*}
% \begin{equation}\label{eq_h2}
% \cdot E\left[\sum_{j}\sum_{i\in\chi(j)}d(x,x'_j(t)) ^{-\alpha}u_{i}(t)\right]=
% \end{equation}
As we assume the base station has utilization $\frac{\bar{\tau}_u}{\tau_u^0}$ in the uplink, and as we have already accounted for the relative duration of the BS time dedicated to each user in \eref{eq:ratio}, we have that
\[
u(x'_i(t))=\frac{1}{\lambda_u A_j}\frac{\bar{\tau}_u}{\tau_u^0}
\]
where $A_j$ is the area of the Voronoi cell of BS j.
Given that users are uniformly distributed in the plane, the palm expectation of \eref{eq:palminterf} is well approximated by 

\[
 \frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}E\left[\sum_{j}\frac{\int_{x'\in A_j} d(x,x')^{-\alpha} dx'}{\lambda_u A_j}\right]\frac{\bar{\tau}_u}{\tau_u^0}=
\]
where $A_j$ is the area of the Voronoi cell of BS j. One can see that $A_j$ is statistically independent on $d(x,x')$. Thus 
the approximated formula becomes
\[
 =\frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}\frac{\int_0^{+\infty}\lambda_u min(1,s^{-\alpha})2\pi s ds}{\lambda_u \bar{A}}\frac{\bar{\tau}_u}{\tau_u^0}
 % E\left[\sum_{j}\frac{\int_{x'\in j} d(x,x')^{-\alpha} dx'}{\lambda_u A_j}\right]=
\]
where $\bar{A}$ is the mean area of a Voronoi cell for a BS density of $\lambda_b$, which is equal to $\lambda_b^{-1}$.
% We can approximate the fraction by considering an equivalent user at the center of the Voronoi cell:
% \[
% =E\left[\sum_{j}d(r_j)^{-\alpha}\right]=
% \]
% where $d(r_j)$ is the distance of the user at $x$ from the $j-th$ base station.
%Similarly to the derivation of the interefering power, and 

Assuming $\alpha>2$, we get
\[
 =\frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}\frac{\lambda_b\frac{\lambda_u 2\pi  }{\alpha-2}}{\lambda_u }\frac{\bar{\tau}_u}{\tau_u^0}=
 \]
 
\[
 =\frac{(1-\gamma)\delta_u P_{bb} +\gamma P_I}{(1-\gamma)\delta_u+\gamma}\frac{\lambda_b \pi \alpha}{\alpha-2}\frac{\bar{\tau}_u}{\tau_u^0}
\]
% \vspace{-0.2in}
% \be\label{eq:interfpower2} 
% =\int_0^{+\infty}\lambda_b min(1,s^{-\alpha})2\pi s ds=\frac{\lambda_b\pi \alpha }{\alpha-2}
% \ee
%where $\lambda_b2\pi sds$ is the mean number of BSs in an annulus of radii $s$ and $s+ds$.
\end{proof}


==> misc-old/03.1.model1.tex <==
\begin{lemma}\label{lemma:perjouledelay} The \textit{ideal per-Joule delay} of a user at $x$ is  given by 
% \begin{equation*}
%   h(x)=\frac{1}{\xi K(x)}\Bigg[P_{BS} D(x)^{-\alpha}\Bigg(G+L\frac{(1-\eta)}{\eta}\bigg)+\bigg.
%  \end{equation*}
% \be
% \left. +\frac{(1-\eta)}{\eta}(I_T(D(x)) +H(x))\right]^{-1}
% \ee
\begin{equation*}
  h(x)=\frac{1}{\xi}\Bigg\{P_{BS} D(x)^{-\alpha}\left[G K(x)+L\left(1-K(x)\frac{(1-\eta)}{\eta}\right)\right]+\bigg.
 \end{equation*}
\be\label{eq:perjoule_delay}
\left. +\left(1-K(x)\frac{(1-\eta)}{\eta}\right)(I(D(x),1) +H(x))\right\}^{-1}
\ee


with 
\[
K(x)=\frac{\frac{\delta_d\eta}{1-\eta}}{N_u(S(x))+\frac{\delta_d}{1-\eta} N_d(S(x))}
\]
\end{lemma}
For the proof, please refer to Appendix \ref{app:proof_lemma_perjouledelay}.
$\xi$ is a factor which accounts for the several technological factors affecting the efficiency of the energy harvesting process, ranging from receiver antenna gain to position and exposure of the specific IoT device, only to mention a few. $I_T(D(x))$ is the interfering power received by considering all base stations, and it is thus independent from reuse factor.  


A measure of system load (or utilization) of a BS is typically the fraction of BS resources (channels, or BS time) which are active.
In what follows we model BS utilization as the average fraction of time in which the BS is transmitting\footnote{thus, we only consider downlink utilization. Indeed, resources consumed in uplink affect very marginally BS power consumption, and they are typically neglected in any BS energy model.}. When transmit power and/or BS service time are higher than that required to achieve the target QoS for information and power transfer,
%threshold expected per-bit delay for both classes of users and the expected transferred energy, 
BSs reduce the amount of time in which they are active, in order to serve users only for the fraction of time required to satisfy the performance constraints of both services, and remaining thus idle (i.e., not transmitting to any user) for the rest.
We model such idle time by introducing a dummy user, with GPS weight $\mu\geq 0$.

Given the considerations made, from the definition of BS utilization we have that its expression, for the BS serving a user at x, is given by 
\[
U(S(x))=\frac{N_u(S(x))+\frac{\delta_d}{1-\eta} N_d(S(x))}{N_u(S(x))+\frac{\delta_d}{1-\eta} N_d(S(x))+\mu}
\]
i.e. by the ratio between the sum of the GPS weights for all active users, over the sum of the weights of all active users and of the dummy user, for that BS.
\footnote{\com{AS uplink does not affect power consumption, BS do not modulate their utilization, i.e. they work always at utilization 1. Thus we do not need the expression of utilization in uplink. This however opens an issue when IoT traffic is considered, because its imbalance towards upload makes sleep mode decisions taken only on downlink inadequate.}}

As explained, the way in which we model energy proportionality in BS is by assuming that each base station modulates $\mu$ and $\eta$ in real time (and thus the amount of base station time dedicated to each of the two categories of users, and to each service)\footnote{do IoT users need to know $\mu$, i.e when to stop listening to info? As energy harvesting is what they do whenever they are not receiving info....} in such a way as to have the average per bit delays and the average per-joule delay \com{(the actual ones, not the ideal ones)} coincide with their respective target values. When this is done, the fraction of time dedicated to the dummy user is the time during which the base station is not active, and thus consuming less power (according to the model in section XX).



More specifically, given the definition of ideal per-bit/per-Joule delay, this is achieved by letting $\mu$ and $\eta$ take values that satisfy the following equations:
\[
\frac{1}{N_{u}(S(x))+\delta_d N_{d}(S(x))}\left (\sum_{x\in\mathcal{X}_{u}}\tau_d(x)\mathbf{1}_{S(x) = S(0)}+\right .
\]
\begin{equation}\label{eq:cond1}
\left .+\delta_d\sum_{x\in\mathcal{X}_{d}}\tau_{d,I}(x)\mathbf{1}_{S(x) = S(0)}\right)\frac{1}{\bar{\tau}_d^0} = U(S(0))
\end{equation} 
% \begin{equation*}
% \frac{\sum_{x\in\mathcal{X}_d}\tau_d(x)}{N_d(S(x))}\mathbf{1}_{S(x) = S(0)} =\bar{\tau}_{d}^0U(S(0))
% \end{equation*} 
\begin{equation}\label{eq:cond2}
\frac{1}{\bar{h}_0}\sum_{x\in\mathcal{X}_d}\frac{h(x)}{N_d(S(x))}\mathbf{1}_{S(x) = S(0)} = U(S(0))
\end{equation}

A measure of utilization is the ratio between the mean performance perceived by the user when all BS resources are employed, and the target mean user performance which is enough to satisfy the user QoS requirements. Indeed, when the former is better than the latter, the ratio between the two performance parameters coincides with the mean fraction of BS resources which are required to deliver the target mean user performance.
In our system, we have three target performance parameters in downlink, of which two are related by $\delta_d=\frac{\bar{\tau}^{0}_{d}}{\bar{\tau}_{d,I}}$, by which it is easy to see that $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{\tau}_{d,I}}{\bar{\tau}^{0}_{d,I}}$. 

As for the mean per joule delay, we note that it is a function of the parameter $\eta$.
Thus the fraction $\frac{\bar{h}}{\bar{h}^{0}}$ is also a function of $\eta$, and thus it is generally not equal to $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}$. As a result, by modulating $\eta$ we also change the mean amount of resources which are required to deliver the target mean per joule delay, in a way which generally does not coincide with the mean fraction of BS resources required to deliver the target user  performance in communication.

impose that 
\[
\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{h}}{\bar{h}^{0}}
\]
 where $\bar{\tau}_d$ and $\bar{h}$ are the ideal per-bit delay of broadband users in downlink and the ideal per-joule delay perceived by the typical user who is beginning service. This condition allows 



%%%%%%
% \[
% \sum_{x\in\mathcal{X}_{u}}\frac{\tau_d(x)}{N_u(S(x))+\frac{\delta_d}{1-\eta} N_d(S(x))}\mathbf{1}_{S(x) = S(0)}+
% \]
% \begin{equation}\label{eq:cond1}
% +\frac{\delta_d}{1-\eta} \sum_{x\in\mathcal{X}_{d}}\frac{\tau_{d,I}(x)}{N_u(S(x))+\frac{\delta_d}{1-\eta} N_d(S(x))}\mathbf{1}_{S(x) = S(0)} =\bar{\tau}_u^0 U(S(0))
% \end{equation} 
% % \begin{equation*}
% % \frac{\sum_{x\in\mathcal{X}_d}\tau_d(x)}{N_d(S(x))}\mathbf{1}_{S(x) = S(0)} =\bar{\tau}_{d}^0U(S(0))
% % \end{equation*} 
% \begin{equation}\label{eq:cond2}
% \sum_{x\in\mathcal{X}_d}\frac{h(x)}{N_d(S(x))}\mathbf{1}_{S(x) = S(0)} =\bar{h}_0 U(S(0))
% \end{equation}


Where $\mathcal{X}_{u}$ and $\mathcal{X}_d$ are the set of broadband and of IoT users, respectively.
They both derive from imposing that the utilization be equal to the ratio between the sample average of the ideal per bit (resp. per-Joule) delay experienced by all users, and the target value. Having both expressions (5) and (6) coincide with base station utilization  
%\footnote{This is only one of the possible ways in which a SWIPT base station can work in order to optimize its resources utilization by bringing it to the minimum value satisfying the QoS targets. Among the many, we chose this as it facilitates the analysis.}
% \[
% \bar{P} U(S(x)) =\bar{P}_0
% \]

\bt[Average BS utilization]\label{th:utilization} For a given density of users, and of base stations, the average base station utilization in the network $\bar{U}$ is given by
%\vspace{-0.3in}
%\vspace{-0.1in}
\begin{eqnarray}\label{eq:utilization_theorem}
\bar{U}=\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{h}}{\bar{h}^{0}}\end{eqnarray}

 where $\bar{\tau}_d$ and $\bar{h}$ are the ideal per-bit delay of broadband users in downlink and the ideal per-joule delay perceived by the typical user who is beginning service. 
% when IoT devices work in the power split mode, and 
% %\vspace{-0.1in}
% \begin{eqnarray}\label{eq:utilization2}
% U(\bar{\tau})=\frac{\bar{\tau}}{\bar{\tau}^{0}}
% \end{eqnarray}
% for the time split model.
\et
For the proof, please refer to Appendix \ref{app:proof_th_utilization}. Note that since we have assumed $\delta_d=\frac{\bar{\tau}^{0}_{d}}{\bar{\tau}_{d,I}}$,
 we have that $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{\tau}_{d,I}}{\bar{\tau}^{0}_{d,I}}$



==> misc-old/07.1.sota.tex <==
\section{Related Works}
\com{Greatly expand, drawing a bit from the intro.}\\
The stochastic geometry is a mathematical study of random spatial patterns, where a key subject is consisted by random point patterns. The current literature is rich of applications of such a theory for the study and analysis of wireless, cellular and ad-hoc network, such that the following surveys and tutorial have been published~\cite{sharma2021resource,amodu2019relay,elsawy2016modeling,okegbile2021stochastic,lu2021stochastic,hmamouche2021new}. All these past experiences have in common that stochastic geometry methods are used to model partial statistical property-based performance parameters (interference, throughput, etc.). Such models can be exploited to study and resolve different challenged related to wireless, cellular, and ad-hoc networks, such as node or user position, user association, state control, power measurements, etc.




==> name.tex <==
A BS tunes its utilization by modulating the amount of BS time dedicated to each class of users, and to energy transfer (by tuning $\delta_{idle}$ and $\eta$), in such a way as to achieve the target QoS for both information and power transfer, for all the classes of users.
%threshold expected per-bit delay for both classes of users and the expected transferred energy, 
%BSs reduce the amount of time in which they are active, in order to serve users only for the fraction of time required to satisfy the performance constraints of both services, and remaining thus idle (i.e., not transmitting to any user) for the rest.
%We model such idle time by introducing a dummy user, with GPS weight $\mu\geq 0$.

A measure of utilization is the ratio between the mean performance perceived by the user when all BS resources are employed, and the target mean user performance which is enough to satisfy the user QoS requirements. Indeed, when the former is better than the latter, the ratio between the two performance parameters coincides with the mean fraction of BS resources which are required to deliver the target mean user performance.
In our system, we have three target performance parameters in downlink, of which two are related by $\delta_d=\frac{\bar{\tau}^{0}_{d}}{\bar{\tau}_{d,I}}$, by which it is easy to see that $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{\tau}_{d,I}}{\bar{\tau}^{0}_{d,I}}$. 

As for the mean per joule delay, we note that it is a function of the parameter $\eta$.
Thus the fraction $\frac{\bar{h}}{\bar{h}^{0}}$ is also a function of $\eta$, and thus it is generally not equal to $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}$. As a result, by modulating $\eta$ we also change the mean amount of resources which are required to deliver the target mean per joule delay, in a way which generally does not coincide with the mean fraction of BS resources required to deliver the target user  performance in communication.

impose that 
\[
\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{h}}{\bar{h}^{0}}
\]
 where $\bar{\tau}_d$ and $\bar{h}$ are the ideal per-bit delay of broadband users in downlink and the ideal per-joule delay perceived by the typical user who is beginning service. This condition allows 


% Where $\mathcal{X}_{u}$ and $\mathcal{X}_d$ are the set of broadband and of IoT users, respectively.
% They both derive from imposing that the utilization be equal to the ratio between the sample average of the ideal per bit (resp. per-Joule) delay experienced by all users, and the target value. Having both expressions (5) and (6) coincide with base station utilization  


\bt[Average BS utilization]\label{th:utilization} For a given density of users, and of base stations, the average base station utilization in the network $\bar{U}$ is given by
%\vspace{-0.3in}
%\vspace{-0.1in}
\begin{eqnarray}\label{eq:utilization_theorem}
\bar{U}=\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{h}}{\bar{h}^{0}}\end{eqnarray}

 where $\bar{\tau}_d$ and $\bar{h}$ are the ideal per-bit delay of broadband users in downlink and the ideal per-joule delay perceived by the typical user who is beginning service. 

\et
For the proof, please refer to Appendix \ref{app:proof_th_utilization}. Note that since we have assumed $\delta_d=\frac{\bar{\tau}^{0}_{d}}{\bar{\tau}_{d,I}}$,
 we have that $\frac{\bar{\tau}_d}{\bar{\tau}^{0}_d}=\frac{\bar{\tau}_{d,I}}{\bar{\tau}^{0}_{d,I}}$




==> note.tex <==
 
\bt[Mean ideal per-bit and per-Joule delay]\label{th:BE_tau} The mean ideal per-bit delays $\bar{\tau}_d$, and the mean ideal per-Joule delay $\bar{h}$ perceived by a typical best-effort user joining the system are given by:
\begin{equation}\label{eq:Poisson}
    \bar{\tau}_d =\int_0^{\infty} f(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{\bar{C}(r,P_{BS},G)}   \diff r.
\end{equation}

\begin{equation}\label{eq:perjoule2}
    \bar{h} =\int_0^{\infty} \frac{f(r)e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{\xi[P_{BS} r^{-\alpha}((G-L)\frac{\delta_d\bar{\eta}}{1-\bar{\eta}}+L)+(k\bar{I}(r,k) +\bar{H}(r))]}   \diff r
\end{equation}

with
\[
f(r)=\int_0^{\infty} \int_0^{2 \pi} 
e^{- \lambda_b A(r, x, \theta)} \lambda_{u}\left[1-\gamma\left(1-\frac{\delta_d}{1-\bar{\eta}}\right)\right] x d \theta d x 
\]
 $A(r, x, \theta)$ is the area of the circle centered at $(x, \theta)$ with radius $x$ that is not overlapped by the circle centered at $(0, -r)$ with radius $r$. $\bar{C}(r)$ is given by \eref{eq:shannon}, with the interference term given by $\bar{I}(r,k)$.

% \begin{equation}\label{eq:perjoule}
%     \bar{h} =\frac{1-\bar{\eta}}{\bar{\eta}}\bar{h}_m 
% \end{equation}

where $\bar{\eta}$ and $\bar{\delta}_{idle}$ are given by the solution of the following fixed point problem:
\[
\frac{\bar{h}(\bar{\eta})}{h_0}=\frac{\bar{N}(\bar{\eta})}{\bar{N}(\bar{\eta})+\bar{\delta}_{idle}}
\]
\be\label{eq:system}
\frac{\bar{\tau}_d(\bar{\eta})}{\tau_d^0}=\frac{\bar{N}(\bar{\eta})}{\bar{N}(\bar{\eta})+\bar{\delta}_{idle}}
\ee
with
\begin{equation}\label{eq:neta}
    \bar{N}(\bar{\eta}) =\int_0^{\infty} f(r)e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \diff r.
\end{equation}
\et

For the proof, please refer to appendix \ref{app:proof_th_BE_tau}.
%\textbf{Does the system $\eref{eq:system}$ admit a single solution?}

%\textbf{Does the system $\eref{eq:system}$ admit a single solution?}

\bt[Mean ideal per-bit and per-Joule delay - uplink]\label{th:BE_tau_uplink} The mean ideal per-bit delay in uplink $\bar{\tau}_u$,  perceived by a typical best-effort user joining the system are given by:
\begin{equation}\label{eq:Poisson_2}
    \bar{\tau}_u =\int_0^{\infty} g(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{\bar{C}(r,P_{I},1)}   \diff r.
\end{equation}
\[
g(r)=\int_0^{\infty} \int_0^{2 \pi} 
e^{- \lambda_b A(r, x, \theta)} \lambda_{u}\left[1-\gamma\left(1-\delta_u\right)\right] x d \theta d x 
\]
$\bar{C}(r,P_{I},1)$ is given by \eref{eq:shannon}, with the interference term equal to zero.
$\bar{\beta}_{idle}$ is given by 
\be\label{eq:beta}
\bar{\beta}_{idle}=\bar{M}\left(\frac{\tau_u^0}{\bar{\tau}_u}-1\right) 
\ee
with
\begin{equation}\label{eq:neta_up}
    \bar{M} =\int_0^{\infty} g(r)e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r \diff r.
\end{equation}
\et



% Similarly, for bb users in the uplink we have 
% \be\label{eq:taubroadband}
% \tau_u(x)=\frac{N_{bb}(S(x))+\delta_u N_{iot}(S(x))}{C(x,P_{bb},1)}
% \ee
% where $P_{bb}$ is the transmit power of broadband users, which are supposed to use no beamforming. 
% For IoT users in uplink, we have 
% \[
% \tau_{u,I}(x)=\frac{N_{bb}(S(x))+\delta_u N_{iot}(S(x))}{\delta_u C(x,P_{iot},1)}
% \]
% where $P_{iot}$ is the transmit power of IoT users.

% While, for IoT users, we have 
% \[
% U_I(x)=\frac{\delta_u}{N_{bb}(S(x))+\delta_u N_{iot}(S(x))}
% \]

% For uplink, formulas are (please correct)
% \be\label{eq:taubroadband_uplink}
% \tau_u= \int_0^{\infty} f(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{\bar{C}(r,P_{bb},1)}   \diff r.
% \ee
% \be\label{eq:taubroadband_uplink}
% \tau_{u,I}= \int_0^{\infty} f(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{\delta_d\bar{C}(r,P_{I},1)}   \diff r.
% \ee






%Note that the expression of $\bar{\tau}$ from \thref{th:BE_tau} is implicit due to the dependency of the interference on the mean BS utilization, which in turn depends on the mean per-bit delay $\bar{\tau}$ through \eref{eq:interfpower}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section we consider the case in which the network only serves best effort users, i.e. $\gamma=0$. We characterize the per-bit delay perceived by a typical best-effort user who is just beginning service,
% as a function of the density of users and base stations under the different base station topologies. 
% \bt\label{th:BE_tau}When $\gamma=0$, the average per-bit delay $\bar{\tau}_{BE}$ 
% perceived by a typical best-effort user joining the system when the density of base stations is $\lambda_b$ 
% and the density of users is $\lambda_u$, and transmit power is $P_T$
% %and the only traffic on the network is the best-effort traffic of a fraction $\gamma$ of the users 
% is given by:
% \begin{eqnarray}\bar{\tau}_{BE} =\int_0^{\infty} f(r)\frac{e^{- \lambda_b \pi r^2} \lambda_b 2 \pi r}{C(r,k)}   d r.
% \end{eqnarray}\label{eq:Poisson} 
% with
% \[
% f(r)=\int_0^{\infty} \int_0^{2 \pi} 
% e^{- \lambda_b A(r, x, \theta)} \lambda_{u} x d \theta d x 
% \]
% where $A(r, x, \theta)$ is the area of the circle centered at $(x, \theta)$ with radius $x$ that is not overlapped by the circle centered at $(0, -r)$ with radius $r$.
% $C(r,k)$ is the capacity to a user at a distance $r$, for a reuse factor $k$, given by
% \be
% C(r,k)=(B/k) \log_{2}\left(1 + \frac{P_Tr^{-\alpha}}{N_0+I(r,k)}\right)
% \ee
% with 
% \be
% I(r,k)=\frac{P_T\lambda_b2\pi r^{2-\alpha}}{k(\alpha-2)}
% \ee
% \et
% For the proof, please refer to \sref{app:proof_tau}.\\
% The following result provides a link between user performance and base station utilization, under the mixed traffic model. 
% \bt\label{th:utilization} For a given density of users, of base stations, and a given share of voice users $\gamma$, the average base station utilization in the network, in the mixed traffic model, is given by
% %\vspace{-0.3in} 
% \[
% U(\lambda_b,\lambda_u,P_T)=\left[1+\gamma\left(R_{0}\frac{\mu_H^{-1}}{\mu_H^{-1}+\mu_W^{-1}}\bar{\tau}^{0}-1\right)\right]
% \]
% \be\label{eq:utilization}
% \frac{\bar{\tau}_{BE}(\lambda_b,\lambda_u,P_T)}{\bar{\tau}^{0}}
% \ee
%  where $\bar{\tau}_{BE}$ is given by \thref{th:BE_tau}.
% \et
% Moreover, it is easy to verify that $U\leq 1 \Rightarrow \bar{\tau}\leq\bar{\tau}^{0}$, where $\bar{\tau}$ is the expected per bit delay for best effort users in the mixed traffic case.\\
% \textbf{cosa accade per $\gamma>0$?}





Fatto:
\begin{itemize}
    \item Cond di convergenza su $\eta$;
    \item Formula esatta (saturata) dell' interferenza. Nota che il modello della bs con pause e' un modello fittizio, quindi in realta' non ci sono pause. Oppure trova come far convergere....
\end{itemize}


Issues:
\begin{itemize}
    \item come fanno i devices a conoscere il $\eta$ usato dalla BS che li serve?
    \item comm limited / power limited capacity regions?
    \item impact of densification on performance
    \item impact on polices for optimal planning/deployment. Increasing P benefits EH (linearly) much more than capacity (through an exponential).
    Hence optimal schemes (what is optimal to do) change! Likely prevalence of sleep modes over P tuning.
    \item add time splitting
    \item queuing: stabilito un arrival rate (inferiore al throughput medio dato come performance target) alcune code restano saturate, altre invece piu' veloci restano inattive, diminuendo l'utilizzazione media delle BS.
    Cambia il calcolo dell' utilizzazione.
    
    \item queuing 2: La mobilita' aiuta la stabilita' del sistema: Se accade, la condizione di coverage basata sulla stabilita (modello con assunzioni diverse) diventa piu' lasca. E piu' ci si muove, inferiore e' il buffer necessario.
    Vedi paper Ayesta: Lo ha gia' detto lui?
    
    \item mobility improves capacity, but not mean rates? However, it should improve harvested energy.
    
    
    \item add beamforming?
    \item universal frequency reuse if you do not play on k!
    \item BS e user clustering
    \item guardati lopez -perez (meo) effetto nlos/los transition!!!
    \item more BSs than users!!! (see lopez)
   %\item slicing (service model)
\end{itemize}

==> numerical_v1.tex <==
\section{Numerical evaluation}
\label{sec:numerical}
%In section xx we have proposed an approach for deriving the energy-optimal configuration of a set of base stations, as a function of BS utilization, of BS transmit power, of BS density, and of user density. It is based on modeling the complex interplay between transmit power, interference, BS utilization and BS consumed power for a same target average user performance. 
In this section, we apply our approach to investigate numerically the performance of different strategies for energy efficiency in cellular access networks.

\subsection{System setup}

Base stations work at a frequency of $1$ GHz, and use a bandwidth of $10$ MHz. We use a log distance path loss model, with path loss at a reference distance of one meter calculated using Friis equation, and with a path loss exponent 
$\alpha = 3$. %\textbf{$(3.5)$?}. %We assume that the rate perceived by users is given by Shannon's capacity law. 
Unless otherwise specified, we consider the case of pure best effort traffic (i.e. $\gamma=0$), and  $\lambda_{b,max}=\infty$.
Note however that from the expression of BS utilization in \thref{eq:utilization} descends that varying $\gamma$ has the same effect on the energy-optimal configuration as a change in the values of the coefficients of the BS energy model.
Finally, in all scenarios we assume user density to vary within a given range $(\lambda_{u}^{min},\lambda_{u}^{max})$. Unless otherwise stated, we set $\lambda_{u}^{max}=0.1$ users per square meter.\\ % \textbf{(reasonable? taken from where?)}\\
We consider two different types of BSs. Namely, macro (with $p_{max}=10$W), and small cell (with $p_{max}=0.13$W). With reference to Table $I$, for each BS type we consider two choices of parameters for the energy models. A first one reflects the behavior of the majority of present day installed BSs \cite{desset2012flexible,imranenergy}, and it is characterized by a low/moderate load proportionality. A second choice of parameters, labeled load proportional or "LP", reflects the load proportionality achievable through time-domain duty-cycling, i.e. through micro-sleep techniques which deactivate some BS components for short time periods \cite{desset2012flexible,futureproof2015}). These techniques, nowadays rarely implemented, make $P_{BB}$ and $P_{RF}$ dependent on load, in a way that increases the overall load dependency of both macro BS and small cell BS. As we can see, such "futuristic" energy models bring the load proportionality (i.e., the percentage of maximum total consumed power which depends on BS load) of both types of BS to about $90\%$. 
%However, we can also observe that, for a same utilization and transmit power, small cells consume an order of magnitude less power than macro cells.\\
%From Table $1$ we can observe that, without micro-sleep techniques, macro BS are much more load proportional than small cell BS. 
%and  (labeled LP) which assumes that various techniques of micro-sleep are in place, leading to a high degree of load proportionality \cite{futureproof2015}.  
%Coherently with \cite{desset2012flexible}, we assume that the ratio between max transmit power and max consumed power, as well as the ratio between $k_1$ and the max consumed power, to be the same for the two types of BSs. We also assume that the power amplifier consumes $60\%$ of total consumed power in both BS types.  
%As a consequence, the dependency of the energy model on utilization and transmit power (what we call "load proportionality") is the same for both BS types. That is, the ratio between the power consumed by a MBS and SCBS for a same couple $(p,U)$ does not vary when varying $(p,U)$.\\
%\begin{center}
\begin{table}
\fontsize{11}{9}
\centering
{\small
    \begin{tabular}{| l | l | l | l | l | l |}\hline
   \textbf{Parameter}     & \multicolumn{2}{| c |}{\textbf{Macro BS}} & \multicolumn{3}{| c |}{\textbf{Small Cell BS}}\\ 
        & Typ & LP & Typ & LP & CRAN\\ \hline
   $p_{min}$ [W] & \multicolumn{2}{| c |}{$0.1$} & \multicolumn{3}{| c |}{$0.001$}\\ \hline
   $p_{max}$ [W] & \multicolumn{2}{| c |}{$10$} & \multicolumn{3}{| c |}{$0.13$}\\ \hline
   Max cons. power [W]& \multicolumn{2}{| c |}{$1500$} & \multicolumn{2}{| c |}{$20$}& $10.6$\\ \hline
   Load proportionality ($\%$)& $60$ & $90$ & $29$& $90$ & $90$\\ \hline
   $P_{PA}$ ($\%$)&\multicolumn{2}{| c |}{$60$} & \multicolumn{2}{| c |}{$29$} & $54.7$\\ \hline %of power consumed by amplifier 
   $P_{BB}$ ($\%$) & \multicolumn{2}{| c |}{$13$} &  \multicolumn{2}{| c |}{ $47$}& $0$\\ \hline  %$\%$ of power consumed by baseband processing
   $k_1$ [W] & $600$ &  $150$  & $14.2$  & $2$ &  $1.06$ \\ \hline
   $k_2$ [W] & $0$ &  $450$ & $0$ &  $12.2$ &  $3.54$ \\ \hline
   $k_3$ [$W^{-1}$]& \multicolumn{2}{| c |}{$90.909$} & \multicolumn{3}{| c |}{$44.961$} \\ \hline
  \end{tabular}
    \caption{\small{Parameters of the energy model of Macro BS and Small Cell BS (\cite{desset2012flexible,imranenergy,futureproof2015}).}}}
\end{table}\label{table1_energymodels2}
%
\begin{figure}[!t]
\includegraphics[width = 3.5in, height= 2.25in]{figures/consumption_macro.pdf}\caption{Power per $km^2$ consumed with the five joint strategies, as a function of user density, for macro BSs.}
\label{f1_macro_powercons}
\end{figure}
%
\begin{figure}[!t]
\includegraphics[width = 3.5in, height= 2.25in]{figures/consumption_sc_new.pdf}\caption{Power per $km^2$ consumed with the five joint strategies, as a function of user density, for small cell BSs.}
\label{f2_small_powercons}
\end{figure}
%
\begin{figure}[!t]
\vspace{-0.2in}
\centering
\includegraphics[width = 3in]{figures/txpower_macro_new.pdf}\caption{Optimal transmit power vs user density, for macro BS.}
\vspace{-0.1in}
\label{f3_txpower_macro}
\end{figure}
%
\begin{figure}[!t]
\centering
\includegraphics[width = 3in]{figures/txpower_sc_new.pdf}\caption{Optimal transmit power vs user density, for small cell BS.}
\vspace{-0.1in}
\label{f4_txpower_small}
\end{figure}
%
\begin{figure}
%\hfill
\centering
\subfigure[Small Cell BS]{\includegraphics[width=3in]{figures/utilization_sc.pdf}}
%\hfill
\subfigure[Macro BS]{\includegraphics[width=3in]{figures/utilization_macro_nolegend.pdf}}
%\hfill
\caption{Optimal BS utilization vs user density.}\label{fig:utilization}
\vspace{-0.2in}
\end{figure}
%In figure xx we have plotted for a MBS and SCBS the values taken by $P_{tot}$ as a function of BS utilization, from \cite{desset2012flexible}. The red curves show the dependency of $P_{tot}$ on the percentage of active subcarriers, and they represent the load proportionality which is common in present day base stations, achieved without putting to sleep any component of the BS. 
%\end{center}%\label{table1_energymodels}
%\subsubsection{Energy models: Futuristic vs actual}
%Available techniques for BS load proportionality are based on a modular BS design, enabling the deactivation of part of the BS components (or on introducing some form of sleep or micro sleep mode, in which such components temporarily enter a state of low power consumption). The result is a power model in which the parameters which have the largest impact on total consumed power are the number of channels used, the fraction of base station time in which the BS transmits, and transmit power.
%Power amplification typically accounts for the largest share of the total consumed power (around $55\%$ in macro BS and $45\%$ in femto BS \cite{desset2012flexible}).   
%In fig xx we have plotted some power consumption curves as a function of transmit power, and of utilization, for macro and femto, based on measured data from \cite{desset2012flexible}. 
%Typically, in macrocells $p$ is around $10W$ and it rarely goes above $20 W$, due to legal and environmental constraints \cite{imranenergy,desset2012flexible,futureproof2015}.
% In traditional BS architectures, dependency of consumed power on load is moderate (around $40\%$ for MBS, and typically around $20\%$ for SBS \textbf{CITE}). However, in 5G scenarios where available techniques for micro-sleeping and other device-level load proportionality techniques are in place, a much more load proportional behavior %(e.g. $91\%$ for macro BS and $11.7\%$ for femto in \cite{desset2012flexible}) 
% can be attained. this can be seen in \fref{fig:macromodel} and \ref{fig:scmodel}, where we have plotted the energy model for 5G SBS and MBS from \cite{desset2012flexible}. For both BS types the power amplifiers accounts for around $60\%$ of total power consumption, and where micro-sleep techniques and transmit power tuning is able to bring to a minimum consumed power which is about $90\%$ the maximum power consumed at full load and at maximum transmit power. 
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/Macro_EM2.pdf}\caption{Energy model for Macro BS, with PA accounting for $60\%$ of total power consumption. Max power consumed is $1500W$. $k_1=100$, $k_2=500W$, $h=0.1818$, max TX power is $10 W$. \cite{desset2012flexible} }
% \label{fig:macromodel}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/smallcell_EM2.pdf}\caption{Energy model for small cell BS, with PA accounting for $60\%$ of total power consumption. Max power consumed is $20W$. $k_1=1.33$, $k_2=6.66W$, $h=14.59$, max TX power is $0.13 W$. \cite{desset2012flexible} }
% \label{fig:scmodel}
% \end{figure}
\subsection{Joint planning and management strategies}
In order to assess the maximum energy savings achievable with joint network planning and management strategies, we consider the following parameters:
\begin{itemize}[leftmargin=*]
    \item $\lambda_b^S$ is the BS density resulting as solution of the optimization problem in \sref{sec:optimizing} with $p=p_{max}$ and $\lambda_u=\lambda_{u,max}$; and 
    \item $\lambda_b^{SO}, p^{SO}$ are the BS density and transmission power resulting from solving the optimization problem in \sref{sec:optimizing} with $\lambda_u=\lambda_{u,max}$.
\end{itemize}
In what follows, and based on the structure of the considered energy model, we consider the following five main joint planning/management strategies:

\subsubsection{Static} It is a network planning strategy with no dynamic network management. That is, both the density of active BSs and the transmit power do not change while the network is operating.
We assume transmit power to be equal to max transmit power, as it is typical in present day access networks \cite{Budzisz_survey_14}. As for the density of installed BS, we assume it is equal to $\lambda_b^S$. 
    
\subsubsection{Sleep} In this joint strategy, the density of installed BS is $\lambda_b^{S}$. During network operation, TX power is kept constant at $p_{max}$, while the density of active BSs, for a given mean value of user density is derived from solving the problem in \sref{sec:optimizing} with $p=p_{max}$, at that value of user density.

\subsubsection{Zoom} In this strategy, the density of active BSs does not vary over time, while their transmit power is varied in order to adapt energy consumption to load. We assume that in the planning phase, the derivation of the optimal density of installed BSs assumes that transmit power can be tuned during network operation. Hence, the density of installed BS is $\lambda_b^{SO}$. For any value of user density, the corresponding optimal transmit power is derived from solving the problem in \sref{sec:optimizing} over transmit power only. 

\subsubsection{Sleep+Zoom} In this case, the density of installed BSs is $\lambda_b^{SO}$. During network operation, for a given mean user density, both the density of active BSs and transmit power are set to be equal to the solution of the problem in \sref{sec:optimizing} for that user density.
	%\textcolor{red}{The density of installed BSs coincides with the optimal BS density at peak user density, and it is hence equal to $\lambda_b^{SO}$.}

\subsubsection{Static Optimal} This is also a network planning strategy with no dynamic network management, like 1) above. The density of installed BSs is set to $\lambda_b^{SO}$. % is the one resulting from solving the problem in \sref{sec:optimizing} over both transmit power and BS density for $\lambda_{u}=\lambda_{u}^{max}$. 
The value of transmit power, which is kept constant during network operation, is derived by solving the problem in \sref{sec:optimizing} only over transmit power, assuming $\lambda_b=\lambda_b^{SO}$, over all the interval $(\lambda_{u}^{min},\lambda_{u}^{max})$, and taking the maximum over the interval. The underlying idea is to avoid dynamic network management, taking for both transmit power and for the density of installed BSs, the maximum values assumed by these quantities in the sleep+zoom strategy, for a given interval of user densities. This brings to a conservative configuration for the network, though less conservative than the purely static strategy.
% \subsubsection{Sleep+Zoom} In this strategy, the network configuration is managed dynamically, varying both BS density and transmit power. For any value of user density, the density of active BSs as well as their transmit power is given by the solution of the problem in \sref{sec:optimizing}. The density of installed BSs coincides with the optimal BS density at peak user density, and it is hence equal to $\lambda_b^{SO}$.
%
%And with $\lambda^*_{b,s+z}(\lambda_{u,max})$ we indicate the optimal BS density at peak user density when both sleeping and zooming modes are in place. That is, the BS density which arises from the solution of Problem \ref{Prob:Opt_1} with $\lambda_{u}=\lambda_{u,max}$.
%In Table XX we have reported, for each strategy considered, the network configuration in terms of total density of installed BSs, density of active base stations and BS transmit power. 
% In order to assess these three strategies, we define a
% For a fair evaluation of the three presented strategies, we assume such default network configuration 
% (i.e. the total installed BS density $\lambda_{b,max}$, and the constant transmit power $p_f$)
% is nonetheless optimized for the peak user density in the considered scenario, $\lambda_{u,max}$, with respect to, respectively, $p$ and  $\lambda_b$ (sleep+zoom strategy), $\lambda_b$ (sleep strategy, with $p=p_{max}$), and $p$ (zoom strategy, with $\lambda_b$ equal to the $\lambda_{b,max}$ computed in the sleep+zoom scenario). \textbf{(questo puo' essere cambiato)}\\
%We define the quantity $\lambda_{b,max}$, i.e. . We assume it is given by optimizing over BS density for the peak user density in the considered scenario, $\lambda_{u,max}$.
%%%%%%%%%%%%%%%%
%
%

Note that, being defined on a homogeneous spatial distribution of users and of BSs, and assuming BS density can be varied with continuity (with no switching costs and delays), these strategies are not directly applicable to a realistic scenario. They have been considered because they give an indication of the maximum energy savings achievable through a given network planning/management approach.
% {\color{red}(a not exhaustive but representative group of strategies. teh yra enot real, practical startegies, but represnetative, and guive an ide aof teh maxuimum savings achievable in ideal condition of "flui9d networks, with all BS density and tx power achievable,a nd instantabneous adaptation 8with nod elay nor switching costs() of network co0nfiguration to user density, and uniformity of user distribution, etc.)}

\subsection{Assessment of the joint strategies}
\begin{figure}[!t]
\centering
\includegraphics[width = 3.3in, height= 2.1in]{figures/bsdensity_new.pdf}\caption{Optimal BS density vs user density.}
\label{fig:bsdensity}
\end{figure}
In a first set of evaluations, we have assessed the performance of the five strategies over a range of user densities of $(10, 10^5)$ users per $km^2$, as the typical values commonly considered in the planning phase usually fall within such an interval. In \fref{f1_macro_powercons} and \fref{f2_small_powercons} we have plotted the power consumed per $km^2$ as a function of user density, for the five strategies. First, it is very important to note that the adoption of a small cell BS layout implies a reduction of the energy consumption of 1-2 orders of magnitude, in spite of the increase in the number of necessary BSs of almost one order of magnitude, as we will see later.
Second, as expected, when micro-sleep modes at the device level are in use at BSs, the static strategy is already able to save energy with respect to present day BSs models. However, the explosion of traffic and the consequent network densification foreseen in future 5G networks will push for more energy-efficient solutions. Moreover, we can see that sleep modes, especially when combined with zooming, still enable the largest energy savings, especially at low user densities. Tuning the transmit power, whether combined with sleeping or not, saves energy with respect to the static strategy even at peak user density, as it allows to decrease interference levels and the power inefficiencies it induces.\\ 
As for the static optimal strategies, we can see that it performs almost identically as the zoom strategy, for all user densities and across all BS power models. Both these strategies are overperformed by sleep and sleep+zoom at very low user densities. However, for user densities close to the peak, the static optimal strategy is more energy efficient than both the pure static and the sleep strategies.\\
%%%comment for small cell vs macro
%% comment on stategies
The configuration induced by each strategy can be better understood by Figs. \ref{f3_txpower_macro} and \ref{f4_txpower_small}, which show the optimal transmit power as a function of user density, and Figure \ref{fig:utilization}, for the optimal BS utilization. The energy savings (of around $60\%$ for macro BS) which zoom, zoom+sleep and static optimal strategies exhibit at peak user density are related to the fraction of total power consumed by a BS which is due to the power amplifier. Indeed, at high user densities, zooming acts by minimizing this contribution by reducing transmit power, while keeping a high BS utilization. When user density decreases, zooming acts by decreasing utilization while at the same time increasing transmit power.\\ 
\fref{fig:bsdensity} shows the optimal BS density for the given strategies, as a function of user density. As we can expect, the use of small cells implies much higher BS densities, with differences of up to one order of magnitude. In addition, we see that, when zooming (with or without sleeping) is in place, or when the static ideal strategy is adopted, even the optimal density of installed BS is decreased with respect to the static (or zooming) strategies. This happens because at high user densities the system is dominated by interference, in a way that increasing the transmitted power of all BS has no impact on SINR. Zooming therefore acts by reducing the energy inefficiency due to interference, by decreasing both the density of installed BS and the transmit power at peak user density.\\
% For the sake of comparison, we have also considered the case in which no mechanism for device-level load proportionality is in use. This may corresponds to the old generation of BSs, in which the only load proportionality is determined by the fraction of time that the power amplifier is active. From \fref{f3} we can see that the savings ($60\%$) of the zooming strategy are now identical to those of the static ideal strategy, and that they remain constant at any user density.\\
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/bsdensity_total2.pdf}\caption{Optimal BS density as a function of user density.}
% \label{f6}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/emme2.pdf}\caption{Energy saved WRT the static scheme, as a percentage of the total energy consumed by the static scheme over a day.}
% \label{f7}
% \end{figure}
% For each of the three schemes, we have plotted the amount of energy consumed at each time during the day, for getting indications on the overall performance of each scheme. Moreover, we have looked at the values of transmit power, utilization, and BS density induced by each scheme, in order to better characterize of the optimal solution stemming from each scheme.
% This is of course an ideal scenario. In realistic setups indeed, the estimation of statistics on user density and achieved quality of service (required by our schemes), and the implementation of configuration changes in BSs require a non-negligible amount of time. In addition, such configuration changes have an energy cost, especially when transitioning a BS from off to on and vice versa, as BS are consuming energy during such transition. Finally, in practical settings not all BS densities are feasible. However, such assumption allows deriving some form of upper bounds to the amount of savings achievable by each of the three proposed schemes.\\
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/mplot.pdf}\caption{.}
% \label{fig:1}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/mplot_conspower.pdf}\caption{.}
% \label{fig:2}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/mplot_txpower.pdf}\caption{.}
% \label{fig:3}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/mplot_utilization2.pdf}\caption{.}
% \label{fig:4}
% \end{figure}
%As we have seen, for the on-off model, the utilization in the energy optimal density is always $1$, while for the energy proportional configuration the BS utilization is generally less than one. As it can be seen in \fref{fig:interf_sc_ut},  
%
%\begin{figure}[!t]
%\includegraphics[width = 3.6in, height= 2.25in]{figures/SC_powerpersquarekm.pdf}\caption{Minimum power consumed per $Km^2$ versus user density, for the optimal BS density in \fref{fig:interf_sc}.}
%\label{fig:interf_sc_ut}
%\end{figure} 
% \subsection{Pisa case} 
% We take the Pisa scenario (i.e. bs layout and orientation, and bs aggregate load profile during the day).
%  The area is defined by the surface which is covered by the Voronoi tessellation of the BS, for the set of BS considered.
% We consider users (load) in the whole area as uniformly distributed over time. Load varies over time according to measures.
% We consider a given target tau (one or two values?).
% For dynamic strategies, we assume configuration is changed instantly.
% We compare the four strategies (s, z, s+z, ideal static) in terms of energy saved during one day.
Overall, strategies which put BSs to sleep save energy when the user density is low
(e.g. during night), while strategies which optimize over transmit power have the largest amount of energy saved during traffic peaks, i.e. when the power consumed by the network is at its highest. 
Bottom line, these trends suggest that among the most important factors in determining the best strategy in a given setting are the peak user density, the peak/valley ratio of the temporal traffic profile, and the amount of time in which the traffic is at high and low values.    
%In order to better 

\subsection{Shanghai setup}
As we have seen, the relative performance of the five strategies depends heavily on how traffic varies during the day. Hence, for a more realistic assessment, we have characterized the relative performance of the four schemes when applied to a setup in which daily patterns of user density are taken from a realistic scenario. \cite{xu2017understanding} identifies five different types of cellular traffic profiles, each related to the main activities of the areas which generate it (office, residential, entertainment, transport, and mixed).
We have assumed for each profile the same peak user density of one user per $10m^2$, and a mean per-bit delay of $100kb/s$. \fref{fig:Shanghai} shows the temporal traffic patterns, as well as the energy savings over $24$ hours for a typical working day, with respect to the static policy, for the 4 policies and the 5 traffic patterns.\\
Moreover, in order to take into account the impact of cloud RAN approaches on our strategies, we have considered a cloud RAN small cell power model, derived from the small cell LP model, but in which the baseband processing is performed on a dedicated device instead of the BS (see Table $I$).  
We can first observe that, as expected, the sleep+zoom policy achieves very large savings (between $70\%$ and $85\%$), which largely outperform the sleep strategy. Second, the zoom strategy, which does not involve BS duty cycling, has a better performance than the sleep strategy, in almost all settings, and all the BS types and configurations. Hence, it is possible to adopt strategies which avoid putting BS to sleep (with all associated issues relative to interference management, and to increase of fault rates, bringing to a decrease of service availability due to a shortening of BS lifetime \cite{chiaraviglio2015life}) without compromising on energy efficiency.
Third, the static optimal strategy, which is based only on a network planning which is optimized according to our approach, has savings comparable to the zoom and sleep strategies, while avoiding all the complexities associated with dynamically managing network resources.  
% As we have seen, what matters is a real profile of traffic, ratio peak/valley, and how long it stays at a given traffic level.
% Evaluate 
% Shanghai:
% \begin{figure*}
% \centering
% \begin{subfigure}%{.5\textwidth}
%   %\centering
%   \includegraphics[width=1in]{figures/res.pdf}
%   \caption{Residential}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}%{.5\textwidth}
%   %\centering
%   \includegraphics[width=1in]{figures/office.pdf}
%   \caption{Office}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{A figure with two subfigures}
% \label{fig:test}
% \end{figure*}
\begin{figure*}
%\hfill
\subfigure[Residential]{\includegraphics[width=2.38in, height=1.68in]{figures/res2_new.pdf}}
%\hfill
\subfigure[Office]{\includegraphics[width=2.38in, height=1.68in]{figures/office2.pdf}}
%\hfill
\subfigure[Transport]{\includegraphics[width=2.38in, height=1.68in]{figures/trans2.pdf}}\\
\subfigure[Entertainment]{\includegraphics[width=2.38in, height=1.68in]{figures/ent2_new.pdf}}
%\hfill
\subfigure[Mixed]{\includegraphics[width=2.38in, height=1.68in]{figures/compr2_new.pdf}}
%\hfill
\subfigure[Normalized traffic patterns]{\includegraphics[width=2.38in, height=1.8in]{figures/tprofile2.pdf}}
\caption{Average energy saved over a typical working day by the considered strategies with respect to the static strategy, for five different temporal traffic profiles in the city of Shanghai \cite{xu2017understanding}}\label{fig:Shanghai}
\end{figure*}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/macro_EP.pdf}\caption{.}
% \label{f1}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/macro_EP_savings2.pdf}\caption{.}
% \label{f2}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/macro_OLD_savings2.pdf}\caption{.}
% \label{f3}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/utilization2.pdf}\caption{(rumore dovuto a  granularita')}
% \label{f4}
% \end{figure}
% \begin{figure}[!t]
% \includegraphics[width = 3.6in, height= 2.25in]{figures/txpower2.pdf}\caption{(rumore dovuto a  granularita')}
% \label{f5}
% \end{figure}
% In a new set of numerical evaluations,  The values of user density over the day are derived from measurements (XX) and they refer to a weekday (though very similar considerations can be made for a weekend day). In such a scenario, we have assumed that the dynamic network management schemes (zoom, sleep, and zoom+sleep) vary in real time the network configuration, ensuring that BS density and/or transmit power are always equal to the optimal values derived from solving the problem in \sref{sec:optimizing} for a given user density. In \fref{xx} we have (in xx) the profile of user density, taken from XX, with a peak user density of $0.1$ users per $m^2$, and a minimum user density of YY users per $m^2$.\\ 
%Finally, the static optimal strategy saves $45.5\%$ of the energy consumed by the static strategy over a  day. 

\subsection{Model Validation} 
Finally, in order to assess the impact of the approximations introduced in the derivation of \thref{th:BE_tau} on the accuracy of the model, we have simulated the system for a range of values of user density between $10$ and $10^5$ users per $km^2$, and for base station densities between $0.1$ and $10^3$ BS per $km^2$. Over these ranges of values, we have compared the measured per-bit delay with the value derived from \thref{th:BE_tau}. The simulation values have been measured with a $97\%$ confidence interval of 
$3\%$ of the mean value. As a result, the mean difference between simulation and analysis has always been within $5\%$, and never larger than $8\%$. 
%which shows that the proposed approach is accurate despite the approximations introduced in its derivation.
%\textbf{abbiamo approx media di f di vc con f di media di vc.
%provando che e' un lower bound (siamo pessimisti).
%qui facciamo sim per vedere di quanto.
%}

 

==> old_intro.tex <==
\section{TODO}
\begin{itemize}
    \item Change BS distribution into something more realistic.
    \item Add evaluations on capex/opex and impact of lifetime shortening according to chiaraviglio.
    \item Add all proof details.
    \item better justify all assumptions made.
\end{itemize}




\section{Introduction}
Energy Efficiency in wireless access networks is improving, mostly thanks to the development of more energy parsimonious base station (BS) generations \cite{Budzisz_survey_14}. With the soon-to-come heterogeneous network architectures of 5G, and the consequent increase in capacity through network densification in high traffic areas, many small cells will be deployed, with limited individual energy consumption, but huge total energy demand \cite{lopez2015towards}. 
This environment offers interesting opportunities for energy efficiency through network management, since the dense small cell deployments will be used to support traffic peaks only in some periods of a day.
The two main approaches to energy efficiency through adaptive management of the network capacity are known as base station sleeping and cell zooming \cite{Budzisz_survey_14,Niu2010}. With the term base station sleeping we mean the possibility of activating and deactivating BSs on demand, %so as to modulate capacity according to end user requests. 
while cell zooming consists in adaptively selecting the transmission power of BSs, so as to modify the BS coverage. Of course, both these approaches have a significant impact of the interference pattern. % since a sleeping BS does not interfere with its neighbors, but when the BS is reactivated, interference surges. Similarly, when zooming makes a cell coverage decrease, interference goes down, but when coverage grows, so does interference.
%Besides efforts on device level energy proportionality, the main approach proposed so far for achieving load proportionality at the network level is through base station (BS) duty cycling. By selectively turning off (or to low power state) some base stations, these techniques (also called "sleep modes") aim at adapting the set of active BSs to traffic load, with the goal of making the power consumption of the network proportional to the amount of served traffic. 

Sleep modes have been proposed in many variants, each of which has shown to be able to deliver savings of at least $20-30\%$ in realistic settings \cite{rengarajan2015energy,Budzisz_survey_14}. However, the validity of such estimations of energy savings are limited to the specific algorithm, and to the setting considered. A few works \cite{rengarajan2015energy} have proposed an analytic approach for estimating the overall energy saving potential of sleep modes. However, such estimates do not take into account the effects of interference, which play a crucial role in determining the overall network performance, especially in future ultra-dense scenarios. Moreover, they are based on a simplified power model, which depends only on BS utilization, and does not take into account the complex interplay between transmit power and utilization.
%However, besides the large amount of attention received from the research community, sleep modes have generally not been adopted by MNOs. This is probably due to the several practical issues which they entail (such as the decrease of BS lifetime and of service availability, and the difficulty of estimating the impact of each change in network configuration on interference) and which cannot be address satisfactorily without greatly increasing the complexity of dynamic network management strategies.

Cell zooming algorithms have been proposed \cite{Niu2010}, as a way to adapt to localized increases in traffic demand, as well as a possible approach to compensate for the loss in coverage and capacity due to BS switch off. 

Energy efficient network planning has also been proposed \cite{Budzisz_survey_14,5956699}, typically as a complement to dynamic network management strategies. However the vast majority of existing results are heuristics based on simple, linear power models which typically neglect the complex interplay between these parameters, the effects of interference, and the total power consumed. Existing estimates of energy savings are closely tied to the details of the given algorithm, and of the setup chosen for the assessment. 
%A general assessment of the potential of such approaches for energy savings (and of their relative performance with respect to sleep modes and to other approaches) is still an open issue to date.\\

This issue becomes even more important in future 5G small cells environments, which are typically dominated by interference. Overall, which dynamic BS management strategy holds the largest potential for energy savings is still an open issue.
% Those works are still be valid as first order evaluations on the potential of dynamic network management for energy efficiency. A first limitation is that they do not consider the effects of interference.
% The remaining works propose specific algorithms (heuristics, as in general such optimization problems are not computationally tractable) and asses the savings. Such evaluation are however closely related to the specific heuristic proposed.
% energy model give idea on where we can intervene to save power
%  energy model used for evaluating potential of sleep modes are basic, and based only on tx power and bs density.
%No reasoning on the potential of tuning the BS operating point for energy efficiency is possible in such settings with such results, if interference and load dependency has to be taken into account.
%  However, they are inadequate and suboptimal when it comes to designing practical sleep strategies. 
% This not only because the power consumption model on which they are based is unrealistic, but also because it neglects the potential of jointly tuning the set of active base stations and their transmit power.\\
% Of course, beyond sleep modes, many other system parameters (antenna orientation, etc) could be tuned in order to drive the system into a more load proportional energy consumption regime, but they are second order effects wrt sleep and load dependency.\\
% Moreover, there are a number of serious drawbacks related to sleeping, which have limited its deployment so far.
% \begin{itemize}
% 	\item Effects of interference: Impossibility to predict the consequence on the transmissive conditions of turning on even a single BS, makes it hard to devise practically feasible algorithms.
% 	\item effects of duty cycling on lifetime (hence capex) and on service (network) availability.
% \end{itemize}
% Study of sleep modes have considered only the possibility of turning off base stations, while BS tuning via power control has been typically considered only as a mean to adapt coverage (and capacity) once the sleep decisions have been taken.
% To the best of our knowledge, all works on the potential of sleep modes for energy savings have been done assuming an oversimplified energy model, in which the dependency was either on the amount of active resources at the base station, or on the BS transmit power, but not on both at the same time. Dependency on load has been usually ignored.

In this paper we propose an analytic framework for the assessment of the potential for energy efficiency of several joint network planning and either static or dynamic management strategies, based on stochastic geometry tools, on an approximate but accurate model of interference, and on a detailed, measurement-driven power model.
More specifically, for a given user density, we propose an approach for deriving the optimal BS density and the BS transmit power which minimize the mean power consumption of the network, while achieving a target QoS level.
Through numerical evaluations, we show the potential savings enabled by joint (and disjoint) optimization of transmit power and density of active BSs. On a realistic setting with measurement-based traffic profiles, we show that huge energy savings are achievable by combining the sleeping and zooming approaches. In addition, we also show that a static strategy, based on carefully planning the density of installed BSs and their transmit power alone reaps most of the benefits of capacity tuning through either sleeping or zooming. This is a result which can have very high relevance for network operators, since it allows them to avoid the feared decrease in operational lifetime (and thus a reduced network availability) which the daily switching of the operational state of BS entails \cite{chiaraviglio2015life}. 
Our results are bounds with respect to what can be actually achieved in real cellular networks, since we assume that any base station density is achievable, although this is clearly not possible in practice.

The paper is organized as follows. In \sref{model} we present the system model, and in \sref{sec:model} we derive a model for user perceived performance. In \sref{sec:optimizing} we formulate an optimization problem for the derivation of the energy optimal network configuration. In \sref{sec:numerical} we assess numerically our results, and in \sref{sec:concl} we conclude the paper.
%Though such models could still be valid to draw first order evaluations on the potential of sleep modes, they are inadequate and suboptimal when it comes to designing practical sleep modes strategies. This not only because the model adopted is unrealistic, but also because it neglects the potential of jointly tuning the set of active base stations and their transmit power.




